UniFormer: Unifying Convolution and Self-attention for Visual Recognition

It is a challenging task to learn discriminative representation from images and videos, due to large local redundancy and complex global dependency in these visual data. Convolution neural networks (CNNs) and vision transformers (ViTs) have been two dominant frameworks in the past few years. Though CNNs can efficiently decrease local redundancy by convolution within a small neighborhood, the limited receptive field makes it hard to capture global dependency. Alternatively, ViTs can effectively capture long-range dependency via self-attention, while blind similarity comparisons among all the tokens lead to high redundancy. To resolve these problems, we propose a novel Unified transFormer (UniFormer), which can seamlessly integrate the merits of convolution and self-attention in a concise transformer format. Different from the typical transformer blocks, the relation aggregators in our UniFormer block are equipped with local and global token affinity respectively in shallow and deep layers, allowing to tackle both redundancy and dependency for efficient and effective representation learning. Finally, we flexibly stack our UniFormer blocks into a new powerful backbone, and adopt it for various vision tasks from image to video domain, from classification to dense prediction. Without any extra training data, our UniFormer achieves 86.3 top-1 accuracy on ImageNet-1K classification. With only ImageNet-1K pre-training, it can simply achieve state-of-the-art performance in a broad range of downstream tasks, e.g., it obtains 82.9/84.8 top-1 accuracy on Kinetics-400/600, 60.9/71.2 top-1 accuracy on Sth-Sth V1/V2 video classification, 53.8 box AP and 46.4 mask AP on COCO object detection, 50.8 mIoU on ADE20K semantic segmentation, and 77.4 AP on COCO pose estimation. We further build an efficient UniFormer with 2-4x higher throughput. Code is available at https://github.com/Sense-X/UniFormer.

==> tables/ablation.tex <==

\begin{table*}[tp]
    \begin{minipage}[t]{1\linewidth}
    	\centering
        \setlength\tabcolsep{6pt}
        \resizebox{\textwidth}{!}{
    	\begin{tabular}{cccc|cccc|cccc}
            \Xhline{0.6pt}
    		\multirow{2}*{Unified} & \multirow{2}*{Joint} & \multirow{2}*{DPE} & \multirow{2}*{Type} & \multicolumn{4}{c|}{ImageNet} & \multicolumn{4}{c}{K400 1$\times$4} \\
    		~ & ~ & ~ & ~ & GFLOPs & \#Param & Top-1 & Top-5 & GFLOPs & \#Param & Top-1 & Top-5 \\
            \Xhline{0.6pt}
            \rowcolor{gray!20} \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & $\mathbf{LLGG}$ &3.6 & 21.5 & \textbf{82.9} & \textbf{96.2} & 41.8 & 21.4 & \textbf{79.3} & \textbf{94.3} \\
    		\hline
    		\XSolidBrush & \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \color{gray}{$\mathrm{LLGG}$} & 3.3 & 21.3 & 82.6 & 96.1 & 41.0 & 21.3 & 78.6 & 93.6 \\
    		\color{lightgray}{\CheckmarkBold} & \XSolidBrush & \color{lightgray}{\CheckmarkBold} & \color{gray}{$\mathrm{LLGG}$} & 3.6 & 21.5 & 82.9 & 96.2 & 36.8 & 27.7 & 78.7 & 94.1 \\ \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \XSolidBrush & 
    		\color{gray}{$\mathrm{LLGG}$} & 3.6 & 21.5 & 82.4 & 96.0 & 41.4 & 21.3 & 77.6 & 93.5 \\
    		\hline
    		\color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & $\mathbf{LLLL}$ & 3.7 & 23.3 & 81.9 & 95.9 & 31.6 & 23.7 & 77.2 & 92.9 \\
    		\color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & $\mathbf{LLLG}$ &  3.7 & 22.2 & 82.5 & 96.1 & 31.6 & 22.4 & 78.4 & 93.3 \\
    		\color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & $\mathbf{LGGG}$ &  3.6 & 21.6 & 82.7 & 96.1 & 39.0 & 21.4 & 79.0 & 94.1 \\
    		\color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & \color{lightgray}{\CheckmarkBold} & $\mathbf{GGGG}$ &  3.7 & 20.1 & 82.1 & 95.9 & 72.0 & 19.8 & 75.3 & 92.4 \\
            \Xhline{0.6pt}
    	\end{tabular}
        }
        \subcaption{\textbf{Structure design.} All models are trained for 50 epochs on Kinetics-400. To guarantee the parameters and computation of all the models are similar, when modifying the stage types, we modify the stage numbers and reduce the computation of self-attention as MViT \cite{mvit} for $\mathrm{LGGG}$ and $\mathrm{GGGG}$.}
        \label{ablation_structure}
        \vspace{1.5mm}
    \end{minipage}
    \begin{minipage}[t]{0.21\linewidth}
    	\centering
        \setlength\tabcolsep{4.5pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}[t]{c|cc}
            \Xhline{0.8pt}
            \multirow{2}*{Size} & IN-1K & K400 \\
            ~ & Top1 & Top1 \\
            \Xhline{0.8pt}
            3 & 82.8 & 79.0 \\
            \rowcolor{gray!20} 5 & \textbf{82.9} & \textbf{79.3} \\
            7 & \textbf{82.9} & 79.1 \\
            9 & 82.8 & 78.9 \\
            \Xhline{0.8pt}
        \end{tabular}
        }
        \subcaption{\textbf{Tube size.} Our network is basically robust to the tube size.}
        \label{ablation_tube}
    \end{minipage}
    \hspace{0.3mm}
    \ 
    \begin{minipage}[t]{0.457\linewidth}
    	\centering
        \setlength\tabcolsep{4.5pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}[t]{cc|c|c|c}
            \Xhline{0.8pt}
            Type & Joint & GFLOPs & Pretrain & SSV1 Top-1 \\
            \Xhline{0.8pt}
        	\multirow{2}*{$\mathbf{LLLL}$} &  \multirow{2}*{\CheckmarkBold} & \multirow{2}*{26.1} & ImageNet & 49.2 \\
        	~ & ~ & ~ & K400 & 49.2\color[RGB]{198, 40, 40}{$(+0.0)$} \\
        	\hline
        	\multirow{2}*{$\mathbf{LLGG}$} &  \multirow{2}*{\XSolidBrush} & \multirow{2}*{36.8} & ImageNet & 51.9 \\
        	~ & ~ & ~ & K400 & 51.8\color[RGB]{198, 40, 40}{$(-0.1)$} \\
        	\hline
            \rowcolor{gray!20} 
            ~ & ~ & ~ & ImageNet & 52.0 \\
            \rowcolor{gray!20} 
        	\multirow{-2}*{$\mathbf{LLGG}$} &  \multirow{-2}*{\CheckmarkBold} & \multirow{-2}*{41.8} & K400 & \textbf{53.8}\color[RGB]{17, 122, 101}{$\mathbf{(+1.8)}$} \\
        % 	~ & ~ & ~ & K600 & \textbf{54.4}\color[RGB]{17, 122, 101}{$\mathbf{(+2.4)}$} \\
            \Xhline{0.8pt}
        \end{tabular}
        }
        \subcaption{\textbf{Transfer learning.} Jointly manner performs better.}
        \label{ablation_tranfer}
    \end{minipage}
    \hspace{0.3mm}
    \ 
    \begin{minipage}[t]{0.308\linewidth}
    	\centering
        \setlength\tabcolsep{2.0pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}[t]{c|c|l|cc}
            \Xhline{0.8pt}
            Dataset & Pretrain & \#Frame & 2D & \cellcolor{gray!20}{3D} \\
            \Xhline{0.8pt}
            \multirow{2}*{K400} & \multirow{2}*{IN-1K} & 8$\times$1$\times$1 & 74.7 & \cellcolor{gray!20}{\textbf{74.9}} \\
            ~ & ~ & 8$\times$1$\times$4 & \textbf{78.5} & \cellcolor{gray!20}{78.4} \\
            \hline
            \multirow{4}*{SSV1} & \multirow{2}*{IN-1K} & 8$\times$1$\times$1 & 47.9 & \cellcolor{gray!20}{\textbf{48.3}} \\
            ~ & ~ & 8$\times$3$\times$1 & \textbf{51.4} & \cellcolor{gray!20}{51.3} \\
            \cline{2-5}
            ~ & \multirow{2}*{K400} & 8$\times$1$\times$1 & 47.9 & \cellcolor{gray!20}{\textbf{48.6}} \\
            ~ & ~ & 8$\times$3$\times$1 & 51.3 & \cellcolor{gray!20}{\textbf{51.5}} \\
            \Xhline{0.8pt}
        \end{tabular}
        }
        \subcaption{\textbf{Inflating method.} Inflating to 3D is better.}
        \label{ablation_inflate}
    \end{minipage}
    % \vspace{1mm}
    \vspace{-0.2cm}
    \caption{\textbf{Ablation studies.} `Unified' means whether to use our local MHRA (\XSolidBrush means to use MobileNet block). `Joint' means whether to use joint attention. `$\mathrm{L}$'/`$\mathrm{G}$' means local/global MHRA.
    `1$\times$4' means multi-clip testing.
    % All video models are trained with 16 frames except the models in Table \ref{ablation_inflate}.
    All video models are trained with 16 frames by defaults.
    }
    \vspace{-0.3cm}
    \label{ablation}
\end{table*}


==> tables/ablation_adaption_detection.tex <==
\begin{table}[tp]
	\centering
    \centering
    \setlength\tabcolsep{1.0pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[t]{c|c|cccc|cccc}
            \Xhline{1.0pt}
            \multirow{2}*{Type} & FLOPs & \multicolumn{4}{c|}{1$\times$ + MS} & \multicolumn{4}{c}{3$\times$ + MS}\\
            ~ & (G) & $AP^b$ & $AP^b_{50}$ & $AP^m$ & $AP^m_{50}$ & $AP^b$ & $AP^b_{50}$ & $AP^m$ & $AP^m_{50}$ \\
            \Xhline{1.0pt}
            W-14 & 250 & 45.0 & 67.8 & 40.8 & 64.7 & 47.5 & 69.8 & 43.0 & 66.7 \\
            \rowcolor{gray!20} 
            H-14 & 269 & 45.4 & 68.2 & 41.4 & 64.9 & \textbf{48.2} & \textbf{70.4} & \textbf{43.4} & \textbf{67.1} \\
            G & 326 & \textbf{45.8} & \textbf{68.7} & \textbf{41.5} & \textbf{50.5} & 48.1 & 70.1 &  \textbf{43.4} & \textbf{67.1} \\
            \Xhline{1.0pt}
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{Adaption types for object detection.}
    \label{ablation_adaption_detection}
    \vspace{-0.3cm}
\end{table}  

==> tables/ablation_adaption_pose.tex <==
\begin{table}[tp]
	\centering
    \centering
    \setlength\tabcolsep{1.5pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[t]{c|c|c|cccccc}
            \Xhline{1.0pt}
            \multirow{2}*{Type} & Input & FLOPs & \multirow{2}*{$AP$} & \multirow{2}*{$AP^{50}$} & \multirow{2}*{$AP^{75}$} & \multirow{2}*{$AP^M$} & \multirow{2}*{$AP^L$} & \multirow{2}*{$AR$} \\
            ~ & Size & (G) & ~ & ~ & ~ & ~ & ~ & ~ \\
            \Xhline{1.0pt}
            W-14 & 384$\times$288 & 12.3 & \textbf{76.1} & 90.8 & 83.2 & \textbf{68.9} & \textbf{79.1} & 81.1 \\
            H-14 & 384$\times$288 & 12.0 & 75.9 & 90.7 & 83.2 & 68.6 & 78.9 & 81.0 \\
            \rowcolor{gray!20} 
            G & 384$\times$288 & 11.1 & 75.9 & 90.6 & \textbf{83.4} & 68.6 & 79.0 & \textbf{81.4} \\
            \Xhline{1.0pt}
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{Adaption types for pose estimation. Due to zero padding, the models with window UniFormer style require more computation. }
    \label{ablation_adaption_pose}
    \vspace{-0.3cm}
\end{table}  

==> tables/ablation_adaption_segmentation.tex <==
\begin{table}[tp]
	\centering
    \centering
    \setlength\tabcolsep{3.0pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[t]{c|c|cc|cc}
            \Xhline{1.0pt}
            \multirow{2}*{Model} & \multirow{2}*{Type}  & \multicolumn{2}{c|}{Semantic FPN} & \multicolumn{2}{c}{UperNet}\\
            ~ & ~ & GFLOPs & mIoU(\%) & GFLOPs & (MS)mIoU(\%) \\
            \Xhline{1.0pt}
            \multirow{4}*{Small} & \color{gray}{H-14} & \color{gray}{190} & \color{gray}{46.3} & \color{gray}{947} & \color{gray}{46.9(48.0)} \\
            ~ & W-32 & 183 & 45.2 & 939 & 46.6(48.4) \\
            ~ & \cellcolor{gray!20}{H-32} & \cellcolor{gray!20}{199} & \cellcolor{gray!20}{46.2} & \cellcolor{gray!20}{955} & \cellcolor{gray!20}{47.0(\textbf{48.5})}  \\
            ~ & G & 247 & \textbf{46.6}& 1004 & \textbf{47.6(48.5)}  \\
            \hline
            \multirow{4}*{Base} & \color{gray}{H-14} & \color{gray}{328} & \color{gray}{47.0} & \color{gray}{1085} & \color{gray}{48.9(50.0)} \\
            ~ & W-32 & 310 & 47.2 & 1066 & 49.1(50.6) \\
            ~ & \cellcolor{gray!20}{H-32} & \cellcolor{gray!20}{350} & \cellcolor{gray!20}{47.7} & \cellcolor{gray!20}{1106} & \cellcolor{gray!20}{49.5(50.7)}  \\
            ~ & G & 471 & \textbf{48.0} & 1227 & \textbf{50.0(50.8)}  \\
            \Xhline{1.0pt}
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{Adaption types for semantic segmentation.}
    \label{ablation_adaption_segmentation}
    \vspace{-0.3cm}
\end{table}  

==> tables/ablation_inflate.tex <==
\begin{table}[tp]
	\centering
    \setlength\tabcolsep{3.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{c|c|c|cc|cc}
        \Xhline{1.0pt}
        \multirow{2}*{Dataset} & \multirow{2}*{Pretrain} & \#frame$\times$ & \multicolumn{2}{c|}{2D} & \multicolumn{2}{c}{\cellcolor{gray!20}{3D}} \\
        ~ & ~ & \#crop$\times$\#clip & Top-1 & Top-5 & \cellcolor{gray!20}{Top-1} & \cellcolor{gray!20}{Top-5} \\
        \Xhline{1.0pt}
        \multirow{2}*{K400} & \multirow{2}*{IN-1K} & 8$\times$1$\times$1 & 74.7 & \textbf{90.8} & \cellcolor{gray!20}{\textbf{74.9}} & \cellcolor{gray!20}{90.7} \\
        ~ & ~ & 8$\times$1$\times$4 & \textbf{78.5} & 93.2 & \cellcolor{gray!20}{78.4} & \cellcolor{gray!20}{\textbf{93.3}} \\
        \hline
        \multirow{4}*{SSV1} & \multirow{2}*{IN-1K} & 8$\times$1$\times$1 & 47.9 & 75.8 & \cellcolor{gray!20}{\textbf{48.3}} & \cellcolor{gray!20}{\textbf{76.1}}  \\
        ~ & ~ & 8$\times$3$\times$1 & \textbf{51.4} & 79.6 & \cellcolor{gray!20}{51.3} & \cellcolor{gray!20}{\textbf{79.7}} \\
        % \cline{2-7}
        \hhline{~|-|-|-|-|-|-}
        ~ & \multirow{2}*{K400} & 8$\times$1$\times$1 & 47.9 & 75.6 & {\cellcolor{gray!20}}{\textbf{48.6}} & {\cellcolor{gray!20}}{\textbf{75.6}} \\
        ~ & ~ & 8$\times$3$\times$1 & 51.3 & 79.4 & \cellcolor{gray!20}{\textbf{51.5}} & \cellcolor{gray!20}{\textbf{79.5}} \\
        \Xhline{1.0pt}
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Inflating methods of convolutional filters.} Inflating the filters to 3D performs better for different datasets.}
    \label{ablation_inflate}
    \vspace{-0.4cm}
\end{table}  

==> tables/ablation_transfer.tex <==
\begin{table}[tp]
    \centering
    \setlength\tabcolsep{2.5pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[t]{c|c|c|cc|c|c}
            \Xhline{1.0pt}
        	\multirow{2}*{Type} & \multirow{2}*{Joint} & \multirow{2}*{GFLOPs} & \multicolumn{2}{c|}{Pretrain} & \multicolumn{2}{c}{SSV1} \\
        	~ & ~ & ~ & Dataset & Top-1 & Top-1 & Top-5 \\
            \Xhline{0.8pt}
        	\multirow{2}*{$\mathbf{LLLL}$} &  \multirow{2}*{\CheckmarkBold} & \multirow{2}*{26.1} & IN-1K & 81.0 & 49.2 & 77.4 \\
        	~ & ~ & ~ & K400 & 77.4 & 49.2\color[RGB]{198, 40, 40}{$(+0.0)$} & 77.6\color[RGB]{17, 122, 101}{$\mathbf{(+0.2)}$} \\
        	\hline
        	\multirow{2}*{$\mathbf{LLGG}$} &  \multirow{2}*{\XSolidBrush} & \multirow{2}*{36.8} & IN-1K & 82.9 & 51.9 & 80.1 \\
        	~ & ~ & ~ & K400 & 80.1 & 51.8\color[RGB]{198, 40, 40}{$(-0.1)$} & 80.1\color[RGB]{198, 40, 40}{$(+0.0)$} \\
        	\hline
            \rowcolor{gray!20} 
            ~ & ~ & ~ & IN-1K & 82.9 & 52.0 & 80.2 \\
            \rowcolor{gray!20} 
        	\multirow{-2}*{$\mathbf{LLGG}$} &  \multirow{-2}*{\CheckmarkBold} & \multirow{-2}*{41.8} & K400 & 80.8 & \textbf{53.8}\color[RGB]{17, 122, 101}{$\mathbf{(+1.8)}$} & \textbf{81.9}\color[RGB]{17, 122, 101}{$\mathbf{(+1.7)}$} \\
        % 	~ & ~ & ~ & K600 & \textbf{54.4}\color[RGB]{17, 122, 101}{$\mathbf{(+2.4)}$} \\
            \Xhline{0.8pt}
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Transfer learning.}
    When the model is gradually pre-trained from ImageNet to Kinetics-400,
    joint manner performs better.}
    \label{ablation_tranfer}
    \vspace{-0.3cm}
\end{table}  

==> tables/more_results_sth.tex <==
\begin{table}[tp]
	\centering
    \setlength\tabcolsep{2pt}
    \resizebox{\linewidth}{!}{
    	\begin{tabular}{c|c|c|c|cc|cc}
            \Xhline{1.0pt}
    		\multirow{2}*{Model} & \multirow{2}*{Pretrain} & \multirow{2}*{\#Frame} & FLOPs & \multicolumn{2}{c|}{SSV1} & \multicolumn{2}{c}{SSV2} \\
    		 ~ & ~ & ~ & (G) & Top-1 & Top-5 & Top-1 & Top-5 \\
            \Xhline{1.0pt}
    		\multirow{12}*{\rotatebox{90}{Small}} & \multirow{3}*{K400} & 16$\times$1$\times$1 & 41.8 & 53.8 & 81.9 & 63.5 & 88.5 \\
    		~ & ~ & 16$\times$3$\times$1 & 125.4 & 57.2 & 84.9 & 67.7 & 91.4 \\
    		~ & ~ & 16$\times$3$\times$2 & 250.8 & 57.3 & 85.1 & 68.1 & 91.7 \\
             \cline{2-8}
    		~ & \multirow{3}*{K600} & 16$\times$1$\times$1 & 41.8 & 54.4 & 81.8 & 65.0 & 89.3 \\
    		~ & ~ & 16$\times$3$\times$1 & 125.4 & 57.6 & 84.9 & 69.4 & 92.1 \\
    		~ & ~ & 16$\times$3$\times$2 & 250.8 & 57.8 & 84.9 & 69.5 & 92.2 \\
             \cline{2-8}
            ~ & \multirow{3}*{K400} & 32$\times$1$\times$1 & 109.6 & 55.8 & 83.6 & 64.9 & 89.2 \\
    		~ & ~ & 32$\times$3$\times$1 & 328.8 & 58.8 & 86.4 & 69.0 & 91.7 \\
    		~ & ~ & 32$\times$3$\times$2 & 657.6 & 58.9 & 86.6 & 69.2 & 91.8 \\
             \cline{2-8}
    		~ & \multirow{3}*{K600} & 32$\times$1$\times$1 & 109.6 & 56.9 & 83.8 & 66.4 & 90.2 \\
    		~ & ~ & 32$\times$3$\times$1 & 328.8 & 59.9 & 86.2 & 70.4 & \textbf{93.1} \\
    		~ & ~ & 32$\times$3$\times$2 & 657.6 & 59.9 & 86.3 & 70.5 & 92.9 \\
            \hline
            \multirow{12}*{\rotatebox{90}{Base}} & \multirow{3}*{K400} & 16$\times$1$\times$1 & 96.7 & 55.4 & 82.9 & 65.8 & 89.9 \\
    		~ & ~ & 16$\times$3$\times$1 & 290.1 & 59.1 & 86.2 & 70.4 & 92.8 \\
    		~ & ~ & 16$\times$3$\times$2 & 580.2 & 59.3 & 86.4 & 70.7 & 92.9 \\
             \cline{2-8}
    		~ & \multirow{3}*{K600} & 16$\times$1$\times$1 & 96.7 & 55.7 & 83.3 & 66.1 & 90.0 \\
    		~ & ~ & 16$\times$3$\times$1 & 290.1 & 58.8 & 86.5 & 70.2 & 93.0 \\
    		~ & ~ & 16$\times$3$\times$2 & 580.2 & 59.1 & 86.5 & 70.7 & 92.9 \\
             \cline{2-8}
            ~ & \multirow{3}*{K400} & 32$\times$1$\times$1 & 259 & 58.1 & 84.9 & 67.2 & 90.2 \\
    		~ & ~ & 32$\times$3$\times$1 & 777 & 60.9 & 87.3 & 71.2 & 92.8 \\
    		~ & ~ & 32$\times$3$\times$2 & 1554 & 61.0 & 87.3 & \textbf{71.4} & 92.8 \\
             \cline{2-8}
    		~ & \multirow{3}*{K600} & 32$\times$1$\times$1 & 259 & 58.0 & 84.9 & 67.5 & 90.2 \\
    		~ & ~ & 32$\times$3$\times$1 & 777 & 61.0 & 87.6 & 71.2 & 92.8 \\
    		~ & ~ & 32$\times$3$\times$2 & 1554 & \textbf{61.2} & \textbf{87.6} & 71.3 & 92.8 \\
            \Xhline{1.0pt}
    	\end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{More results on Something-Something V1\&V2.} Small models are eager for larger dataset pre-training.}
    \label{more_results_sth}
\vspace{-0.3cm}
\end{table}  

==> tables/results_ade.tex <==
\begin{table*}[t]
	\begin{minipage}[t]{0.49\textwidth}
        \centering
        \setlength\tabcolsep{8.7pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}[t]{l|ccc}
            \Xhline{1.0pt}
            \multirow{2}{*}{Method} & \multicolumn{3}{c}{Semantic FPN 80K}\\
             &   \#Param(M) & FLOPs(G) & mIoU(\%) \\ 
            \Xhline{1.0pt}
            Res50 \cite{resnet} & 29 & 183 & 36.7 \\
            PVT-S \cite{pvt} & 28 & 161 & 39.8 \\
            TwinsP-S \cite{twins} & 28 & 162 & 44.3 \\
            Twins-S \cite{twins} & 28 & 144 & 43.2 \\
            Swin-T \cite{swin} & 32 & 182 & 41.5 \\
            \rowcolor{gray!20} 
            UniFormer-S$_{h32}$ & 25 & 199 & \textbf{46.2} \\
            \color{gray}{UniFormer-S} & \color{gray}{25} & \color{gray}{247} & \color{gray}{46.6} \\
            \Xhline{1.0pt}
            Res101 \cite{resnet} & 48 & 260 & 38.8\\
            PVT-M \cite{pvt} & 48 & 219 & 41.6 \\
            PVT-L \cite{pvt} & 65 & 283 & 42.1 \\
            TwinsP-B \cite{twins} & 48 & 220 & 44.9 \\
            TwinsP-L \cite{twins} & 65 & 283 & 46.4 \\
            Twins-B \cite{twins} & 60 & 261 & 45.3 \\
            Swin-S \cite{swin}  & 53 & 274 & 45.2 \\
            \color{gray}{Twins-L \cite{twins}}  & \color{gray}{104} & \color{gray}{404} & \color{gray}{46.7} \\
            \color{gray}{Swin-B \cite{swin}}  & \color{gray}{91} & \color{gray}{422} & \color{gray}{46.0} \\
            \rowcolor{gray!20} 
            UniFormer-B$_{h32}$ & 54 & 350
            & \textbf{47.7} \\
            \color{gray}{UniFormer-B} & \color{gray}{54} & \color{gray}{471} & \color{gray}{48.0} \\
            \Xhline{1.0pt}
        \end{tabular}
        }
        \vspace{-0.2cm}
        \caption{\textbf{Semantic segmentation with semantic FPN on ADE20K.} The FLOPs are measured at resolution 512$\times$2048.
        `$h32$' means we utilize hybrid UniFormer blocks with window size of 32 in Stage3.}
        \label{results_ade_fpn}
    \end{minipage}
    \hspace{2mm}
	\begin{minipage}[t]{0.49\textwidth}
        \centering
        \setlength\tabcolsep{1.5pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}[t]{l|cccc}
            \Xhline{1.0pt}
            \multirow{2}{*}{Method} & \multicolumn{4}{c}{Upernet 160K}\\
             &  \#Param.(M) & FLOPs(G) & mIoU(\%) & MS mIoU(\%) \\ 
            \Xhline{1.0pt}
            TwinsP-S \cite{twins} & 55  & 919  & 46.2 & 47.5 \\
            Twins-S \cite{twins} & 54  & 901  & 46.2 & 47.1 \\
            Swin-T \cite{swin} & 60  & 945  & 44.5 & 45.8 \\
            Focal-T \cite{focal}  & 62  & 998 & 45.8 & 47.0 \\
            Shuffle-T \cite{shuffleTR} & 60 & 949 & 46.6 & 47.8 \\
            \rowcolor{gray!20} 
            UniFormer-S$_{h32}$ & 52 & 955 & \textbf{47.0} & \textbf{48.5} \\
            \color{gray}{UniFormer-S} & \color{gray}{52} & \color{gray}{1008} & \color{gray}{47.6} & \color{gray}{48.5} \\
            \Xhline{1.0pt}
            Res101 \cite{resnet} & 86  & 1029 & - & 44.9 \\
            TwinsP-B \cite{twins} & 74 & 977  & 47.1 & 48.4 \\
            Twins-B \cite{twins} & 89  & 1020 & 47.7 & 48.9 \\
            Swin-S \cite{swin}  & 81 & 1038 & 47.6 & 49.5 \\
            Focal-T \cite{focal} & 85 & 1130 & 48.0 & 50.0 \\
            Shuffle-S \cite{shuffleTR} & 81  & 1044 & 48.4 & 49.6 \\
            \color{gray}{Swin-B \cite{swin}} & \color{gray}{121} & \color{gray}{1188} & \color{gray}{48.1} & \color{gray}{49.7} \\
            \color{gray}{Focal-B \cite{focal}} & \color{gray}{126} & \color{gray}{1354} & \color{gray}{49.0} & \color{gray}{50.5} \\
            \color{gray}{Shuffle-B \cite{shuffleTR}} & \color{gray}{121}  & \color{gray}{1196} & \color{gray}{49.0} & \color{gray}{50.5} \\
            \rowcolor{gray!20} 
            UniFormer-B$_{h32}$ & 80 & 1106 & \textbf{49.5} & \textbf{50.7} \\
            \color{gray}{UniFormer-B} & \color{gray}{80} & \color{gray}{1227} &  \color{gray}{50.0} & \color{gray}{50.8} \\
            \Xhline{1.0pt}
        \end{tabular}
        }
        \vspace{-0.2cm}
        \caption{\textbf{Semantic segmentation with Upernet on ADE20K.} The FLOPs are measured at resolution 512$\times$2048.
        `$h32$' means we utilize hybrid UniFormer blocks with window size of 32 in Stage3.}
        \label{results_ade_upernet}
    \end{minipage}
    \vspace{-0.4cm}
    % \label{results_ade}
\end{table*}
